Attribute-Enhanced Similarity Ranking for Sparse Link Prediction

Link prediction is a fundamental problem in graph data. In its most realistic setting, the problem consists of predicting missing or future links between random pairs of nodes from the set of disconnected pairs. Graph Neural Networks (GNNs) have become the predominant framework for link prediction. GNN-based methods treat link prediction as a binary classification problem and handle the extreme class imbalance -- real graphs are very sparse -- by sampling (uniformly at random) a balanced number of disconnected pairs not only for training but also for evaluation. However, we show that the reported performance of GNNs for link prediction in the balanced setting does not translate to the more realistic imbalanced setting and that simpler topology-based approaches are often better at handling sparsity. These findings motivate Gelato, a similarity-based link-prediction method that applies (1) graph learning based on node attributes to enhance a topological heuristic, (2) a ranking loss for addressing class imbalance, and (3) a negative sampling scheme that efficiently selects hard training pairs via graph partitioning. Experiments show that Gelato outperforms existing GNN-based alternatives.

==> iclr2023/results_tables/hits_bt.tex <==

% \newcommand{\first}[1]{\textcolor{blue}{\textbf{#1}}}
% % Second
% \newcommand{\second}[1]{\textcolor{red}{\textbf{#1}}}
% % Third 
% \newcommand{\third}[1]{\textcolor{brown}{\textbf{#1}}}

\begin{table}
    \setlength\tabcolsep{4.65pt}
    \small
  \caption{We show present results (mean $\pm$ std hits@100) for GNN methods versus Gelato trained in \textit{biased training} splits and evaluated on \textit{unbiased} (Cora and CiteSeer) and \textit{partitioned} (OGBL-DDI) splits.}
  \centering
  \label{tab::ap::hits_bt}%
  \begin{threeparttable}
  % \fontsize{6}{7.2}

    \begin{tabular}{ccccc}
    \toprule
          &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{ogbl-ddi}\\
    \midrule
    & SEAL & \third{1.14} \tnote{*} & \second{2.2} \tnote{*} & \third{0.05} \tnote{*} \\
    & NeoGNN & 0.82 ± 0.11 & \third{1.83 ± 0.34} & \second{0.066} \tnote{*} \\
    & BUDDY & \second{1.52 ± 0.0} & 1.32 ± 0.0 & \second{0.066 ± 0.0} \\
    & NCN & 0.0 ± 0.0 & 0.11 ± 0.16 & 0.0 ± 0.0 \\
    \midrule    
    & Gelato & \first{3.42 ± 0.33} & \first{3.44 ± 0.13} & \first{0.071 ± 0.0} \\
    \bottomrule
    \end{tabular}%
	\begin{tablenotes}[para]
	\item[*] Run only once as each run takes $>$24 hrs.
	% \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
    \end{tablenotes}
    
  \end{threeparttable}
\end{table}





==> iclr2023/results_tables/hits_bt_bt.tex <==
% \begin{table*}[htbp]
% \setlength\tabcolsep{4.65pt}
% \small
% \centering
% \caption{We show results (mean $\pm$ std Hits@100) for Gelato trained and evaluated in the \textit{biased} setting. The top three models are colored by \textcolor{blue}{\textbf{First}}, \textcolor{red}{\textbf{Second}} and \textcolor{brown}{\textbf{Third}}.}
% \label{tab::ap::hits_bt_bt}
% \begin{tabular}{lccc}
% \toprule
% Cora & CiteSeer & DDI \\
% \midrule
% SEAL & 89.18 ± nan & 90.99 ± nan & 4.66 ± nan \\
% NeoGNN & 62.49 ± 9.87 & 89.16 ± 0.83 & 5.22 ± nan \\
% Buddy & 93.36 ± 0.0 & 98.68 ± 0.0 & 0.33 ± 0.0 \\
% NCN & 93.36 ± 0.54 & 95.93 ± 0.47 & 0.76 ± 0.6 \\
% Gelato & 78.49 ± 0.22 & 84.4 ± 0.0 & 4.18 ± 0.0 \\
% \bottomrule
% \end{tabular}
% \end{table*}

% First
\newcommand{\first}[1]{\textcolor{blue}{\textbf{#1}}}
% Second
\newcommand{\second}[1]{\textcolor{red}{\textbf{#1}}}
% Third 
\newcommand{\third}[1]{\textcolor{brown}{\textbf{#1}}}

\begin{table}
    \setlength\tabcolsep{4.65pt}
    \small
  
  \caption{We show results (mean $\pm$ std hits@100) for GNN methods versus Gelato trained in \textit{biased training} splits and evaluated on \textit{unbiased} (Cora and CiteSeer) and \textit{partitioned} (OGBL-DDI) splits. The top three models are colored by \textcolor{blue}{\textbf{First}}, \textcolor{red}{\textbf{Second}} and \textcolor{brown}{\textbf{Third}}.}
  \centering
  \label{tab::ap::hits_bt_bt}%
  \begin{threeparttable}
  % \fontsize{6}{7.2}

    \begin{tabular}{ccccc}
    \toprule
          &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{ogbl-ddi}\\
    \midrule
    
    & SEAL & \second{89.18}\tnote{*}& \third{90.99}\tnote{*}& \second{4.66}\tnote{*}\\
    & NeoGNN & 62.49 ± 9.87 & 89.16 ± 0.83 & \first{5.22}\tnote{*} \\
    & BUDDY & \first{93.36 ± 0.0} & \first{98.68 ± 0.0} & 0.33 ± 0.0\\
    & NCN & \first{93.36 ± 0.54} & \second{95.93 ± 0.47} & 0.76 ± 0.6 \\
    
    \midrule    
    & Gelato & \third{78.49 ± 0.22} & 84.4 ± 0.0 & \third{4.18 ± 0.0} \\
    \bottomrule
    \end{tabular}%
	\begin{tablenotes}[para]
	\item[*] Run only once as each run takes $>$24 hrs.
	% \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
    \end{tablenotes}
    
  \end{threeparttable}
\end{table}



==> iclr2023/results_tables/mrr_bt.tex <==

\begin{table}[htbp]
    \setlength\tabcolsep{4.65pt}
    \small
    \caption{We show present results (mean $\pm$ std MRR) for GNN methods versus Gelato trained in \textit{biased training} splits and evaluated on \textit{unbiased} (Cora and CiteSeer) and \textit{partitioned} (DDI) splits. The top three models are colored by \textcolor{blue}{\textbf{First}}, \textcolor{red}{\textbf{Second}} and \textcolor{brown}{\textbf{Third}}.}
  \centering
  \label{tab::ap::biased_mrr}%
  
  \begin{threeparttable}
  % \fontsize{6}{7.2}
    \begin{tabular}{ccccc}
    \toprule
          &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{ogbl-ddi}\\
    \midrule
    
    & SEAL & \textcolor{brown}{\textbf{0.0637}}\tnote{*} & \textcolor{red}{\textbf{0.1602}}\tnote{*} & \textcolor{brown}{\textbf{0.0067}}\tnote{*} \\
    & NeoGNN & 0.0505 ± 0.0145 & \textcolor{blue}{\textbf{0.2312 ± 0.0796}} & \textcolor{blue}{\textbf{0.0544}}\tnote{*} \\
    & BUDDY & \textcolor{red}{\textbf{0.1776 ± 0.0}} & 0.12 ± 0.0 & 0.0059 ± 0.0 \\
    & NCN & 0.0012 ± 0.0012 & 0.0126 ± 0.0176 & 0.0006 ± 0.0001 \\
    
    \midrule    
    & Gelato & 
    \textcolor{blue}{\textbf{0.2564 ± 0.0069}} & \textcolor{brown}{\textbf{0.1418 ± 0.0011}} & \textcolor{red}{\textbf{0.0084 ± 0.0}}\\
    \bottomrule
    \end{tabular}%
	\begin{tablenotes}[para]
	\item[*] Run only once as each run takes $>$24 hrs.
	% \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
    \end{tablenotes}
    
  \end{threeparttable}
\end{table}






==> iclr2023/results_tables/mrr_bt_bt.tex <==
% \begin{table}[htbp]
%     \setlength\tabcolsep{4.65pt}
%     \small
%   \centering
%   \caption{}
%   \label{tab::ap::mrr_bt_bt}%
%   \begin{threeparttable}
%   % \fontsize{6}{7.2}

%     \begin{tabular}{ccccc}
%     \toprule
%           &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{ogbl-ddi}\\
%     \midrule
%     \multirow{4}[2]{*}{GNN} 
%         & SEAL & 24.4477\tnote{*} & 41.0729\tnote{*} & 0.5548\tnote{*}\\
%         & Neo-GNN & 21.759 ± 12.7653 & 34.8363 ± 3.0621 & 0.3829\tnote{*} \\ 
%         & BUDDY & 35.1812 ± 0.0 & 34.4924 ± 0.0 & 0.0292 ± 0.0\\
%         & NCN & 4.2344 ± 4.5023 & 13.1176 ± 17.5428 & 0.046 ± 0.0084\\
%     \midrule    
%     \multicolumn{2}{c}{Gelato} & 26.9161 ± 0.0 & 54.2946 ± 0.0 & 0.3091 ± 0.0\\
%     \bottomrule
%     \end{tabular}%
% 	\begin{tablenotes}[para]
% 	\item[*] Run only once as each run takes 
% 	\raise.17ex $>$24 hrs.
% 	% \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
%     \end{tablenotes}
    
%   \end{threeparttable}
% \end{table}






==> kdd2024/results_tables/ap.tex <==
% \begin{table}[htbp]
%     \setlength\tabcolsep{4.65pt}
%     \small
%   \centering
%   \caption{Link prediction performance comparison (mean ± std AP) for all datasets considered. Gelato consistently outperforms GNN-based methods, topological heuristics, and two-stage approaches combining attributes/topology. For \textsc{Cora}, \textsc{CiteSeer}, \textsc{ogbl-ddi} and \textsc{PubMed} results we used \emph{unbiased} training, while for \textsc{ogbl-collab} \emph{negative} sampling is used, for scalability reasons}
%   \label{tab::performance_ap}%
%   \begin{threeparttable}
  
%     \begin{tabular}{ccccccc}
%     \toprule
%           &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{PubMed} & \textsc{ogbl-ddi} & \textsc{ogbl-collab} \\
%     \midrule
%     \multirow{5}[2]{*}{GNN} 

%         & SEAL & 2.21\tnote{*} & 2.43\tnote{*} & *** & 35.2\tnote{*} &  \textbf{47.43}\tnote{*}\\
%         & Neo-GNN & 2.15 ± 1.51 & 1.71 ± 0.06 & 1.21 ± 0.14 & 24.42\tnote{*} & 31.86\tnote{*} \\ 
%         & BUDDY & 1.20 ± 0.25 & 1.72 ± 0.08 & OOM & 21.59 ± 1.02 & 47.13 ± 0.22 \\
%         & NCN & 1.82 ± 0.49 & 2.79 ± 0.21 & 0.06 ± 0.07 & 44.75 ± 0.07 & 41.38 ± 0.44 \\
%         & NCNC & 2.88 ± 0.16 & 3.23 ± 0.44 & 1.54 ± 0.01 & \textbf{44.9 ± 0.05} & 27.67 ± 3.3 \\
%     \midrule
%     \multicolumn{1}{c}{\multirow{2}[2]{*}{\parbox{1.8cm}{\centering Topological Heuristics}}} 
%         & CN & 1.10 ± 0.00 & 0.74 ± 0.00 & 0.36 ± 0.00 & 24.76 ± 0.00 & 24.18 ± 0.00 \\
%         & AA & 2.07 ± 0.00 & 1.24 ± 0.00 & 2.50 ± 0.00 & 25.25 ± 0.00 & 34.28 ± 0.00 \\
%         % & RA & 2.02 ± 0.00 & 1.19 ± 0.00 & 0.33 ± 0.00 & 10.77 ± 0.00 \\
%         & AC & 2.43 ± 0.00 & 2.65 ± 0.00 & 2.50 ± 0.00 & 30.75 ± 0.00 & 37.92 ± 0.00\\
%     \midrule
%     % \multicolumn{1}{c}{\multirow{5}[2]{*}{\parbox{1.8cm}{\centering Attributes + Topology}}} 
%     %  & MLP       & 0.30 ± 0.05 & 0.44 ± 0.09 & 0.14 ± 0.06 & 1.01 ± 0.26 & 0.41 ± 0.23 \\
%     %  & Cos       & 0.42 ± 0.00 & 1.89 ± 0.00 & 0.07 ± 0.00 & 0.11 ± 0.00 & 0.07 ± 0.00 \\
%     %  & MLP+AC    & 3.24 ± 0.03 & 1.95 ± 0.05 & 2.61 ± 0.06 & 15.99 ± 0.21 & 11.25 ± 0.13 \\
%     %  & Cos+AC    & 3.60 ± 0.00 & 4.46 ± 0.00 & 0.51 ± 0.00 & 10.01 ± 0.00 & 5.20 ± 0.00 \\
%     %  & MLP+Cos+AC& 3.39 ± 0.06 & 4.15 ± 0.14 & 0.55 ± 0.03 & 10.88 ± 0.09 & 5.75 ± 0.11 \\
%     % \midrule
%     %\multicolumn{2}{c}{Cluster AC} & 2.31 ± 0.00 & 1.54 ± 0.00 & 1.10 ± 0.00     & 6.76 ± 0.00      & 6.09 ± 0.00 \\
%     %\multicolumn{2}{c}{ClusterGelato} & 2.47 ± 0.13 & 2.77 ± 0.08 & 2.53 ± 0.10     & 17.52 ± 0.78      & 9.46 ± 0.16 \\
%     \multicolumn{2}{c}{Gelato} & \textbf{3.90 ± 0.03} & \textbf{4.55 ± 0.02} & \textbf{2.88 ± 0.09} & 29.42 ± 0.09      & 42.53\tnote{*} \\
%     \bottomrule
%     \end{tabular}%
% 	\begin{tablenotes}[para]
% 	\item[*] Run only once as each run takes 
% 	\raise.17ex $>$24 hrs.
% 	% \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
%     \end{tablenotes}
    
%   \end{threeparttable}
% \end{table}



\begin{table}[htbp]
    \setlength\tabcolsep{4.65pt}
    \small
  \centering
  \caption{Link prediction performance comparison (mean ± std AP) for all datasets considered. Gelato consistently outperforms GNN-based methods, topological heuristics, and two-stage approaches combining attributes/topology, being at least in the top-3 best-performing models in all datasets. For \textsc{Cora}, \textsc{CiteSeer}, \textsc{ogbl-ddi} and \textsc{PubMed} results we used \emph{unbiased} training, while for \textsc{ogbl-collab} \emph{partitioned} sampling is used, for scalability reasons. The top three models are colored by \textcolor{blue}{\textbf{First}}, \textcolor{red}{\textbf{Second}} and \textcolor{brown}{\textbf{Third}}.}
  \label{tab::performance_ap}%
  \begin{threeparttable}
  
    \begin{tabular}{ccccccc}
    \toprule
          &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{PubMed} & \textsc{ogbl-ddi} & \textsc{ogbl-collab} \\
    \midrule
    \multirow{5}[2]{*}{GNN} 

        & SEAL & 2.21\tnote{*} & 2.43\tnote{*} & *** & 35.2\tnote{*} &  \textcolor{blue}{\textbf{47.43}}\tnote{*}\\
        & Neo-GNN & 2.15 ± 1.51 & 1.71 ± 0.06 & 1.21 ± 0.14 & 24.42\tnote{*} & 31.86\tnote{*} \\ 
        & BUDDY & 1.20 ± 0.25 & 1.72 ± 0.08 & OOM & 21.59 ± 1.02 & \textcolor{red}{\textbf{47.13 ± 0.22}} \\
        & NCN & 1.82 ± 0.49 & \textcolor{brown}{\textbf{2.79 ± 0.21}} & 0.06 ± 0.07 & \textcolor{red}{\textbf{44.75 ± 0.07}} & 41.38 ± 0.44 \\
        & NCNC & \textcolor{red}{\textbf{2.88 ± 0.16}} & \textcolor{red}{\textbf{3.23 ± 0.44}} & \textcolor{brown}{\textbf{1.54 ± 0.01}} & \textcolor{blue}{\textbf{44.9 ± 0.05}} & 27.67 ± 3.3 \\
    \midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{\parbox{1.8cm}{\centering Topological Heuristics}}} 
        & CN & 1.10 ± 0.00 & 0.74 ± 0.00 & 0.36 ± 0.00 & 24.76 ± 0.00 & 24.18 ± 0.00 \\
        & AA & 2.07 ± 0.00 & 1.24 ± 0.00 & \textcolor{red}{\textbf{2.50 ± 0.00}} & 25.25 ± 0.00 & 34.28 ± 0.00 \\
        % & RA & 2.02 ± 0.00 & 1.19 ± 0.00 & 0.33 ± 0.00 & 10.77 ± 0.00 \\
        & AC & \textcolor{brown}{\textbf{2.43 ± 0.00}} & 2.65 ± 0.00 & \textcolor{red}{\textbf{2.50 ± 0.00}} & \textcolor{brown}{\textbf{29.42 ± 0.00}} & 37.92 ± 0.00\\
    \midrule
    % \multicolumn{1}{c}{\multirow{5}[2]{*}{\parbox{1.8cm}{\centering Attributes + Topology}}} 
    %  & MLP       & 0.30 ± 0.05 & 0.44 ± 0.09 & 0.14 ± 0.06 & 1.01 ± 0.26 & 0.41 ± 0.23 \\
    %  & Cos       & 0.42 ± 0.00 & 1.89 ± 0.00 & 0.07 ± 0.00 & 0.11 ± 0.00 & 0.07 ± 0.00 \\
    %  & MLP+AC    & 3.24 ± 0.03 & 1.95 ± 0.05 & 2.61 ± 0.06 & 15.99 ± 0.21 & 11.25 ± 0.13 \\
    %  & Cos+AC    & 3.60 ± 0.00 & 4.46 ± 0.00 & 0.51 ± 0.00 & 10.01 ± 0.00 & 5.20 ± 0.00 \\
    %  & MLP+Cos+AC& 3.39 ± 0.06 & 4.15 ± 0.14 & 0.55 ± 0.03 & 10.88 ± 0.09 & 5.75 ± 0.11 \\
    % \midrule
    %\multicolumn{2}{c}{Cluster AC} & 2.31 ± 0.00 & 1.54 ± 0.00 & 1.10 ± 0.00     & 6.76 ± 0.00      & 6.09 ± 0.00 \\
    %\multicolumn{2}{c}{ClusterGelato} & 2.47 ± 0.13 & 2.77 ± 0.08 & 2.53 ± 0.10     & 17.52 ± 0.78      & 9.46 ± 0.16 \\
    \multicolumn{2}{c}{Gelato} & \textcolor{blue}{\textbf{3.90 ± 0.03}} & \textcolor{blue}{\textbf{4.55 ± 0.02}} & \textcolor{blue}{\textbf{2.88 ± 0.00}} & \textcolor{brown}{\textbf{29.42 ± 0.00}}      & \textcolor{brown}{\textbf{42.53}}\tnote{*} \\
    \bottomrule
    \end{tabular}%
	\begin{tablenotes}[para]
	\item[*] Run only once as each run takes 
	\raise.17ex $>$24 hrs.
	% \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
    \end{tablenotes}
    
  \end{threeparttable}
\end{table}

==> kdd2024/results_tables/hits.tex <==
% \begin{table}[ht!]
%     \setlength\tabcolsep{4.65pt}
%     \small
%   \centering
%   \caption{Link prediction performance comparison (mean ± std hits@1000) for all datasets considered. Gelato consistently outperforms GNN-based methods, topological heuristics, and two-stage approaches combining attributes/topology. For \textsc{Cora}, \textsc{CiteSeer}, \textsc{ogbl-ddi} and \textsc{PubMed} results we used \emph{unbiased} training, while for \textsc{ogbl-collab} \emph{negative} sampling is used, for scalability reasons}
%   \label{tab::performance_hits}%
%   \begin{threeparttable}
  
%     \begin{tabular}{ccccccc}
%     \toprule
%           &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{PubMed} & \textsc{ogbl-ddi} & \textsc{ogbl-collab} \\
%     \midrule
%     \multirow{5}[2]{*}{GNN} 

%         & SEAL & 0.0\tnote{*} & 7.25\tnote{*} & *** & 0.75\tnote{*} &  25.9\tnote{*}\\
%         & Neo-GNN & 6.96 ± 4.24 & 5.42 ± 0.13 & 1.63 ± 0.32 & 0.76\tnote{*} & 0.85\tnote{*} \\ 
%         & BUDDY & 4.81 ± 0.72 & 5.86 ± 0.34 & OOM & 0.74 ± 0.01 & 27.66 ± 0.24 \\
%         & NCN & 4.11 ± 1.22 & 7.84 ± 1.13 & 0.06 ± 0.1 & 0.82 ± 0.02 & 7.16 ± 1.42 \\
%         & NCNC & 6.58 ± 0.58 & 8.72 ± 2.08 & 1.04 ± 0.09 & \textbf{0.89 ± 0.09} & 0.44 ± 0.37 \\
%     \midrule
%     \multicolumn{1}{c}{\multirow{2}[2]{*}{\parbox{1.8cm}{\centering Topological Heuristics}}} 
%         & CN & 4.17 ± 0.00 & 4.4 ± 0.00 & 0.36 ± 0.00 & 0.8 ± 0.00 & 2.4 ± 0.00 \\
%         & AA & 6.64 ± 0.00 & 4.4 ± 0.00 & 1.13 ± 0.00 & 0.79 ± 0.00 & 4.88 ± 0.00 \\
%         & AC & 11.20 ± 0.00 & 14.29 ± 0.00 & 3.81 ± 0.00 &  0.78 ± 0.00 & 12.89 ± 0.00\\
%     \midrule
%     \multicolumn{2}{c}{Gelato} & \textbf{16.62 ± 0.31} & \textbf{19.78 ± 0.23} & \textbf{4.18 ± 0.19} &  0.78 ± 0.00      & \textbf{30.92}\tnote{*} \\
%     \bottomrule
%     \end{tabular}%
% 	\begin{tablenotes}[para]
% 	\item[*] Run only once as each run takes $>$24 hrs; \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
%     \end{tablenotes}
    
%   \end{threeparttable}
% \end{table}



\begin{table}[ht!]
    \setlength\tabcolsep{4.65pt}
    \small
  \centering
  \caption{Link prediction performance comparison (mean ± std hits@1000) for all datasets considered. Gelato consistently outperforms GNN-based methods, topological heuristics, and two-stage approaches combining attributes/topology. For \textsc{Cora}, \textsc{CiteSeer}, \textsc{ogbl-ddi} and \textsc{PubMed} results we used \emph{unbiased} training, while for \textsc{ogbl-collab} \emph{negative} sampling is used, for scalability reasons. The top three models are colored by \textcolor{blue}{\textbf{First}}, \textcolor{red}{\textbf{Second}} and \textcolor{brown}{\textbf{Third}}.}
  \label{tab::performance_hits}%
  \begin{threeparttable}
  
    \begin{tabular}{ccccccc}
    \toprule
          &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{PubMed} & \textsc{ogbl-ddi} & \textsc{ogbl-collab} \\
    \midrule
    \multirow{5}[2]{*}{GNN} 

        & SEAL & 0.0\tnote{*} & 7.25\tnote{*} & *** & 0.75\tnote{*} &  25.9\tnote{*}\\
        & Neo-GNN & \textcolor{brown}{\textbf{6.96 ± 4.24}} & 5.42 ± 0.13 & \textcolor{brown}{\textbf{1.63 ± 0.32}} & 0.76\tnote{*} & 0.85\tnote{*} \\ 
        & BUDDY & 4.81 ± 0.72 & 5.86 ± 0.34 & OOM & 0.74 ± 0.01 & \textcolor{red}{\textbf{27.66 ± 0.24}} \\
        & NCN & 4.11 ± 1.22 & 7.84 ± 1.13 & 0.06 ± 0.1 & \textcolor{red}{\textbf{0.82 ± 0.02}} & 7.16 ± 1.42 \\
        & NCNC & 6.58 ± 0.58 & \textcolor{brown}{\textbf{8.72 ± 2.08}} & 1.04 ± 0.09 & \textcolor{blue}{\textbf{0.89 ± 0.09}} & 0.44 ± 0.37 \\
    \midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{\parbox{1.8cm}{\centering Topological Heuristics}}} 
        & CN & 4.17 ± 0.00 & 4.4 ± 0.00 & 0.36 ± 0.00 & \textcolor{brown}{\textbf{0.8 ± 0.00}} & 2.4 ± 0.00 \\
        & AA & 6.64 ± 0.00 & 4.4 ± 0.00 & 1.13 ± 0.00 & 0.79 ± 0.00 & 4.88 ± 0.00 \\
        & AC & \textcolor{red}{\textbf{11.20 ± 0.00}} & \textcolor{red}{\textbf{14.29 ± 0.00}} & \textcolor{red}{\textbf{3.81 ± 0.00}} &  0.78 ± 0.00 & 12.89 ± 0.00\\
    \midrule
    \multicolumn{2}{c}{Gelato} & \textcolor{blue}{\textbf{16.62 ± 0.31}} & \textcolor{blue}{\textbf{19.78 ± 0.23}} & \textcolor{blue}{\textbf{4.18 ± 0.19}} &  0.78 ± 0.00      & \textcolor{blue}{\textbf{30.92}}\tnote{*} \\
    \bottomrule
    \end{tabular}%
	\begin{tablenotes}[para]
	\item[*] Run only once as each run takes $>$24 hrs; \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
    \end{tablenotes}
    
  \end{threeparttable}
\end{table}


==> kdd2024/results_tables/hits_bt.tex <==

\begin{table}[htbp]
    \setlength\tabcolsep{4.65pt}
    \small
  \centering
  \caption{We show present results (mean $\pm$ std Hits@100) for GNN methods versus Gelato trained in \textit{biased training} splits and evaluated on \textit{biased} (Cora and CiteSeer) and \textit{partitioned} (DDI) splits. }
  \label{tab::performance_ap}%
  \begin{threeparttable}
  % \fontsize{6}{7.2}

    \begin{tabular}{ccccc}
    \toprule
          &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{ogbl-ddi}\\
    \midrule
    \multirow{4}[2]{*}{GNN} 
    & SEAL & 4.36 \tnote{*} & 7.91 \tnote{*} & 0.71 \tnote{*} \\
    & NeoGNN & 3.1 ± 2.25 & 6.15 ± 0.38 & 0.79 \tnote{*} \\
    & BUDDY & 5.12 ± 0.0 & 4.4 ± 0.0 & 0.55 ± 0.0 \\
    & NCN & 0.0 ± 0.0 & 0.77 ± 1.09 & 0.01 ± 0.01 \\
    \midrule    
    \multicolumn{2}{c}{Gelato} & 12.46 ± 0.29 & 13.77 ± 0.51 & 0.78 ± 0.0 \\
    \bottomrule
    \end{tabular}%
	\begin{tablenotes}[para]
	\item[*] Run only once as each run takes 
	\raise.17ex $>$24 hrs.
	% \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
    \end{tablenotes}
    
  \end{threeparttable}
\end{table}





==> kdd2024/results_tables/hits_bt_bt.tex <==
% \begin{table*}[htbp]
% \setlength\tabcolsep{4.65pt}
% \small
% \centering
% \caption{We show results (mean $\pm$ std Hits@100) for Gelato trained and evaluated in the \textit{biased} setting. The top three models are colored by \textcolor{blue}{\textbf{First}}, \textcolor{red}{\textbf{Second}} and \textcolor{brown}{\textbf{Third}}.}
% \label{tab::ap::hits_bt_bt}
% \begin{tabular}{lccc}
% \toprule
% Cora & CiteSeer & DDI \\
% \midrule
% SEAL & 89.18 ± nan & 90.99 ± nan & 4.66 ± nan \\
% NeoGNN & 62.49 ± 9.87 & 89.16 ± 0.83 & 5.22 ± nan \\
% Buddy & 93.36 ± 0.0 & 98.68 ± 0.0 & 0.33 ± 0.0 \\
% NCN & 93.36 ± 0.54 & 95.93 ± 0.47 & 0.76 ± 0.6 \\
% Gelato & 78.49 ± 0.22 & 84.4 ± 0.0 & 4.18 ± 0.0 \\
% \bottomrule
% \end{tabular}
% \end{table*}


\begin{table}[]
    \setlength\tabcolsep{4.65pt}
    \small
  
  \caption{We show present results (mean $\pm$ std MRR) for GNN methods versus Gelato trained in \textit{biased training} splits and evaluated on \textit{unbiased} (Cora and CiteSeer) and \textit{partitioned} (DDI) splits. The top three models are colored by \textcolor{blue}{\textbf{First}}, \textcolor{red}{\textbf{Second}} and \textcolor{brown}{\textbf{Third}}.}
  \centering
  \label{tab::ap::hits_bt_bt}%
  \begin{threeparttable}
  % \fontsize{6}{7.2}

    \begin{tabular}{ccccc}
    \toprule
          &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{ogbl-ddi}\\
    \midrule
    \multirow{4}[2]{*}{GNN} 
    & SEAL & 89.18\tnote{*}& 90.99\tnote{*}& 4.66\tnote{*}\\
    & NeoGNN & 62.49 ± 9.87 & 89.16 ± 0.83 & 5.22 ± nan\tnote{*} \\
    & BUDDY & 93.36 ± 0.0 & 98.68 ± 0.0 & 0.33 ± 0.0\\
    & NCN & 93.36 ± 0.54 & 95.93 ± 0.47 & 0.76 ± 0.6 \\
    
    \midrule    
    \multicolumn{2}{c}{Gelato} & 78.49 ± 0.22 & 84.4 ± 0.0 & 4.18 ± 0.0 \\
    \bottomrule
    \end{tabular}%
	\begin{tablenotes}[para]
	\item[*] Run only once as each run takes 
	% \raise.17ex $>$24 hrs.
	% \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
    \end{tablenotes}
    
  \end{threeparttable}
\end{table}



==> kdd2024/results_tables/mrr.tex <==

\begin{table}[htbp]
    \setlength\tabcolsep{4.65pt}
    \small
  \centering
  \caption{Link prediction performance comparison (mean ± std MRR). Gelato shows competitive performance, despite its simplicity, being in the top-3 best-performing models in almost all datasets. We highlight that Gelato is the best-performing method in \textsc{PubMed} and \textsc{ogbl-collab}, the hardest evaluation regimes since we consider the \textit{unbiased testing} scenario for both datasets. The top three models are colored by \textcolor{blue}{\textbf{First}}, \textcolor{red}{\textbf{Second}} and \textcolor{brown}{\textbf{Third}}.}
  \label{tab::performance_mrr}%
  \begin{threeparttable}
  % \fontsize{6}{7.2}

    \begin{tabular}{ccccccc}
    \toprule
          &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{PubMed} & \textsc{ogbl-ddi} & \textsc{ogbl-collab} \\
    \midrule
    \multirow{5}[2]{*}{GNN} 
        & SEAL & 0.0204\tnote{*} & 0.235\tnote{*} & *** & 0.0071\tnote{*} &  \textcolor{red}{\textbf{4.9441}}\tnote{*}\\
        & Neo-GNN & 0.2216 ± 0.101 & 0.0969 ± 0.0285 & 0.0001 ± 0.0001 & \textcolor{brown}{\textbf{0.0098}}\tnote{*} & 0.3435\tnote{*} \\ 
        & BUDDY & 0.136 ± 0.0607 & 0.121 ± 0.0026 & OOM & 0.0094 ± 0.0003 & \textcolor{brown}{\textbf{1.2285 ± 0.0576}} \\
        & NCN & 0.1216 ± 0.0551 & \textcolor{red}{\textbf{0.1989 ± 0.0515}} & \textcolor{brown}{\textbf{0.0005 ± 0.0007}} & \textcolor{red}{\textbf{0.0117 ± 0.002}} & 0.1343 ± 0.0588 \\
        & NCNC & \textcolor{blue}{\textbf{0.4606 ± 0.1867}} & \textcolor{blue}{\textbf{0.2934 ± 0.1746}} & 0.0002 ± 0.00004 & \textcolor{blue}{\textbf{0.0171 ± 0.0133}} & 0.011 ± 0.0042 \\
    \midrule
    \multicolumn{1}{c}{\multirow{1}[2]{*}{\parbox{1.8cm}{\centering Topological Heuristics}}} 
        & CN & 0.1816 ± 0.00 & 0.0933 ± 0.00 &  0.0001 ± 0.0000 & 0.0103 ± 0.00 & 0.4767 ± 0.00 \\
        & AA & 0.1764 ± 0.00 & 0.1154 ± 0.00 &  0.0001 ± 0.0000 & 0.0104 ± 0.00 & 0.0333 ± 0.00 \\
        % & RA & 2.02 ± 0.00 & 1.19 ± 0.00 & 0.33 ± 0.00 & 10.77 ± 0.00 \\
        & AC & \textcolor{red}{\textbf{0.3069 ± 0.00}} & 0.1245 ± 0.00 & \textcolor{red}{\textbf{0.0006 ± 0.00}} & 0.0084 ± 0.00 & 0.7692 ± 0.00 \\
    \midrule
    % \multicolumn{1}{c}{\multirow{5}[2]{*}{\parbox{1.8cm}{\centering Attributes + Topology}}} 
    %  & MLP       & 0.30 ± 0.05 & 0.44 ± 0.09 & 0.14 ± 0.06 & 1.01 ± 0.26 & 0.41 ± 0.23 \\
    %  & Cos       & 0.42 ± 0.00 & 1.89 ± 0.00 & 0.07 ± 0.00 & 0.11 ± 0.00 & 0.07 ± 0.00 \\
    %  & MLP+AC    & 3.24 ± 0.03 & 1.95 ± 0.05 & 2.61 ± 0.06 & 15.99 ± 0.21 & 11.25 ± 0.13 \\
    %  & Cos+AC    & 3.60 ± 0.00 & 4.46 ± 0.00 & 0.51 ± 0.00 & 10.01 ± 0.00 & 5.20 ± 0.00 \\
    %  & MLP+Cos+AC& 3.39 ± 0.06 & 4.15 ± 0.14 & 0.55 ± 0.03 & 10.88 ± 0.09 & 5.75 ± 0.11 \\
    % \midrule
    %\multicolumn{2}{c}{Cluster AC} & 2.31 ± 0.00 & 1.54 ± 0.00 & 1.10 ± 0.00     & 6.76 ± 0.00      & 6.09 ± 0.00 \\
    %\multicolumn{2}{c}{ClusterGelato} & 2.47 ± 0.13 & 2.77 ± 0.08 & 2.53 ± 0.10     & 17.52 ± 0.78      & 9.46 ± 0.16 \\
    \multicolumn{2}{c}{Gelato} & \textcolor{brown}{\textbf{0.2558 ± 0.0001}} & \textcolor{brown}{\textbf{0.1424 ± 0.0028}} & \textcolor{blue}{\textbf{0.0009 ± 0.0003}} & 0.0084 ± 0.001      & \textcolor{blue}{\textbf{6.1422}}\tnote{*} \\
    \bottomrule
    \end{tabular}%
	\begin{tablenotes}[para]
	\item[*] Run only once as each run takes 
	\raise.17ex $>$24 hrs.
	% \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
    \end{tablenotes}
    
  \end{threeparttable}
\end{table}

==> kdd2024/results_tables/mrr_bt.tex <==

\begin{table}[]
    \setlength\tabcolsep{4.65pt}
    \small
  
  \caption{We show present results (mean $\pm$ std MRR) for GNN methods versus Gelato trained in \textit{biased training} splits and evaluated on \textit{unbiased} (Cora and CiteSeer) and \textit{partitioned} (DDI) splits. The top three models are colored by \textcolor{blue}{\textbf{First}}, \textcolor{red}{\textbf{Second}} and \textcolor{brown}{\textbf{Third}}.}
  \label{tab::ap::biased_mrr}%
  \centering
  \begin{threeparttable}
  % \fontsize{6}{7.2}

    \begin{tabular}{ccccc}
    \toprule
          &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{ogbl-ddi}\\
    \midrule
    \multirow{4}[2]{*}{GNN} 
    & SEAL & \textcolor{brown}{\textbf{0.0637}}\tnote{*} & \textcolor{red}{\textbf{0.1602}}\tnote{*} & \textcolor{brown}{\textbf{0.0067}}\tnote{*} \\
    & NeoGNN & 0.0505 ± 0.0145 & \textcolor{blue}{\textbf{0.2312 ± 0.0796}} & \textcolor{blue}{\textbf{0.0544}}\tnote{*} \\
    & BUDDY & \textcolor{red}{\textbf{0.1776 ± 0.0}} & 0.12 ± 0.0 & 0.0059 ± 0.0 \\
    & NCN & 0.0012 ± 0.0012 & 0.0126 ± 0.0176 & 0.0006 ± 0.0001 \\
    
    \midrule    
    \multicolumn{2}{c}{Gelato} & 
    \textcolor{blue}{\textbf{0.2564 ± 0.0069}} & \textcolor{brown}{\textbf{0.1418 ± 0.0011}} & \textcolor{red}{\textbf{0.0084 ± 0.0}}\\
    \bottomrule
    \end{tabular}%
	\begin{tablenotes}[para]
	\item[*] Run only once as each run takes 
	\raise.17ex $>$24 hrs.
	% \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
    \end{tablenotes}
    
  \end{threeparttable}
\end{table}





==> kdd2024/results_tables/mrr_bt_bt.tex <==
\begin{table}[htbp]
    \setlength\tabcolsep{4.65pt}
    \small
  \centering
  \caption{}
  \label{tab::ap::mrr_bt_bt}%
  \begin{threeparttable}
  % \fontsize{6}{7.2}

    \begin{tabular}{ccccc}
    \toprule
          &       & \textsc{Cora}  & \textsc{CiteSeer} & \textsc{ogbl-ddi}\\
    \midrule
    \multirow{4}[2]{*}{GNN} 
        & SEAL & 24.4477\tnote{*} & 41.0729\tnote{*} & 0.5548\tnote{*}\\
        & Neo-GNN & 21.759 ± 12.7653 & 34.8363 ± 3.0621 & 0.3829\tnote{*} \\ 
        & BUDDY & 35.1812 ± 0.0 & 34.4924 ± 0.0 & 0.0292 ± 0.0\\
        & NCN & 4.2344 ± 4.5023 & 13.1176 ± 17.5428 & 0.046 ± 0.0084\\
    \midrule    
    \multicolumn{2}{c}{Gelato} & 26.9161 ± 0.0 & 54.2946 ± 0.0 & 0.3091 ± 0.0\\
    \bottomrule
    \end{tabular}%
	\begin{tablenotes}[para]
	\item[*] Run only once as each run takes 
	\raise.17ex $>$24 hrs.
	% \hspace{5pt} *** Each run takes $>$1000 hrs; \hspace{5pt} OOM: Out Of Memory.
    \end{tablenotes}
    
  \end{threeparttable}
\end{table}



==> kdd2024/sec_abstract.tex <==
\begin{abstract}
Link prediction is a fundamental problem in graph data. In its most realistic setting, the problem consists of predicting missing or future links between random pairs of nodes from the set of disconnected pairs. Graph Neural Networks (GNNs) have become the predominant framework for link prediction. GNN-based methods treat link prediction as a binary classification problem and handle the extreme class imbalance---real graphs are very sparse---by sampling (uniformly at random) a balanced number of disconnected pairs not only for training but also for evaluation. However, we show that the reported performance of GNNs for link prediction in the balanced setting does not translate to the more realistic imbalanced setting and that simpler topology-based approaches are often better at handling sparsity. These findings motivate Gelato, a similarity-based link-prediction method that applies (1) graph learning based on node attributes to enhance a topological heuristic, (2) a ranking loss for addressing class imbalance, and (3) a negative sampling scheme that efficiently selects hard training pairs via graph partitioning. Experiments show that Gelato is more accurate and faster than existing GNN-based alternatives.

%TODO: justify negative sampling based on social networks

%Both of these procedures are concerning from the perspective of real-world applications: the intrinsic class imbalance of the problem---due to the graph sparsity---is not leveraged by the balanced negative sampling, and the binary classification perspective of Link Prediction is often not the sustainable, due to the presence of near indistinguishable negative and positive pairs. To address these issues, (i) we propose a novel model-agnostic partitioned negative-sampling technique that enables sampling harder negative pairs, closer to a more realistic scenario, and (ii) a new frame on Link Prediction as a similarity-based problem, justified through theoretical and empirical results. We demonstrate the capabilities of our ideas through \emph{Gelato}, our proof of concept model. \emph{Gelato} is a similarity-based method that applies a topological heuristic to an attribute-enhanced graph, being more robust to class imbalance and using significantly fewer parameters than the GNN-based methods.
%Graph Neural Networks (GNNs), which are based on an attribute-centric message-passing paradigm, became the predominant framework for link prediction (predicting edges based on graph features). Due to the semi-supervised nature of this task, GNN-based methods treat Link Prediction as a binary classification problem, artificially sampling negative pairs of nodes (negative sampling) to balance positive pairs to train and evaluate their performance. Both of these procedures are concerning from the perspective of real-world applications: the intrinsic class imbalance of the problem---due to the graph sparsity---is not leveraged by the balanced negative sampling, and the binary classification perspective of Link Prediction is often not the sustainable, due to the presence of near indistinguishable negative and positive pairs. To address these issues, (i) we propose a novel model-agnostic partitioned negative-sampling technique that enables sampling harder negative pairs, closer to a more realistic scenario, and (ii) a new frame on Link Prediction as a similarity-based problem, justified through theoretical and empirical results. We demonstrate the capabilities of our ideas through \emph{Gelato}, our proof of concept model. \emph{Gelato} is a similarity-based method that applies a topological heuristic to an attribute-enhanced graph, being more robust to class imbalance and using significantly fewer parameters than the GNN-based methods.
\end{abstract}

% JOAO: PREVIOUS VERSION BELOW
% --------
% \begin{abstract}
% %Link prediction is one of the most fundamental problems for graph-structured data. As in other graph-related tasks, Graph Neural Networks (GNNs) are becoming the predominant tool to solve link prediction, and have demonstrated success compared to traditional topology-based heuristics. However, there is little understanding of what contributes to the performance gains. Is that because of the supervised learning scheme, the incorporation of node attributes, or the representational power of the architecture? 
% %This paper provides answers to these questions. We first scrutinize the training and evaluation of GNN-based methods, and identify their key limitations in addressing the class imbalance problem in link prediction. 
% %Next, we propose Gelato, a simple link prediction framework without GNNs that (1) learns to enhance the original graph based on node attributes via a Multi-Layer Perceptron and (2) computes a topological heuristic, Autocovariance, on the enhanced graph for link prediction. To effectively train our model under severe class imbalance, we propose a rank-based link prediction loss and argue for the inclusion of all negative (disconnected) pairs in training. 
% % \looseness=-1
% Link prediction, which consists of predicting edges based on graph features, is a fundamental task in many graph applications. As for several related problems, Graph Neural Networks (GNNs), which are based on an attribute-centric message-passing paradigm, have become the predominant framework for link prediction. GNNs have consistently outperformed traditional topology-based heuristics, but what contributes to their performance? %Is it the potential to discover better topological heuristics via supervised learning or the ability to incorporate node attributes?
% Are there simpler approaches that achieve comparable or better results? To answer these questions, we first identify important limitations in how GNN-based link prediction methods handle the intrinsic class imbalance of the problem---due to the graph sparsity---in their training and evaluation. %Next, we propose Gelato, a simple alternative framework that directly incorporates node attributes into an enhanced graph via a neural network and applies a topological heuristic on it for link prediction.  
% We then propose \emph{Gelato}, a novel topology-centric framework that applies a topological heuristic to a graph enhanced by attribute information via graph learning. \emph{Gelato} is more robust to class imbalance as it requires significantly fewer parameters than the GNN-based alternatives. 
% % via a Multi-Layer Perceptron. 
% %a graph enhanced based on node attribute information.
% Our model is trained end-to-end with an N-pair loss on an unbiased training set to address the class imbalance. Experiments show that Gelato is 84\% more accurate, trains 3 times faster, and infers 10,000 times faster compared to state-of-the-art GNN for link prediction. 
% %Our model is trained end-to-end with an N-pair loss on an unbiased training set to address class imbalance. Experiments show that Gelato is 84\% more accurate, trains 3 times faster, infers 10,000 times faster, and has less than half of the trainable parameters compared to state-of-the-art GNNs for link prediction. \looseness=-1
% \end{abstract}

% %shortened version
% %Link prediction, which aims to predict links/edges based on graph features, is a fundamental task in many graph applications. As for many related problems, Graph Neural Networks (GNNs) have become the go-to framework for link prediction, consistently outperforming traditional topology-based heuristics. However, what contributes to the GNN performance? Is it the ability to incorporate node/edge attributes or the potential to learn better topological heuristics directly from data? To answer these questions, we first identify important limitations in how GNN-based link prediction methods handle the intrinsic class imbalance of the problem in their training and evaluation. We address these limitations by proposing GELATO, a simple link prediction method that combines graph learning, a topological heuristic, and a rank-based loss. Our experiments show that Gelato performs 87.9\% better on average, trains 11 times faster, infers 6,000 times faster, and has less than half the trainable parameters of state-of-the-art GNNs for link prediction.

% %   The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
% %   both the left- and right-hand margins. Use 10~point type, with a vertical
% %   spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
% %   bold, and in point size 12. Two line spaces precede the abstract. The abstract
% %   must be limited to one paragraph.

==> kdd2024/sec_acknowledgement.tex <==
\begin{acks}
To Robert, for the bagels and explaining CMYK and color spaces.
\end{acks}

